Primate Face Identification in the Wild

Ecological imbalance owing to rapid urbanization and deforestation has adversely affected the population of several wild animals. This loss of habitat has skewed the population of several non-human primate species like chimpanzees and macaques and has constrained them to co-exist in close proximity of human settlements, often leading to human-wildlife conflicts while competing for resources. For effective wildlife conservation and conflict management, regular monitoring of population and of conflicted regions is necessary. However, existing approaches like field visits for data collection and manual analysis by experts is resource intensive, tedious and time consuming, thus necessitating an automated, non-invasive, more efficient alternative like image based facial recognition. The challenge in individual identification arises due to unrelated factors like pose, lighting variations and occlusions due to the uncontrolled environments, that is further exacerbated by limited training data. Inspired by human perception, we propose to learn representations that are robust to such nuisance factors and capture the notion of similarity over the individual identity sub-manifolds. The proposed approach, Primate Face Identification (PFID), achieves this by training the network to distinguish between positive and negative pairs of images. The PFID loss augments the standard cross entropy loss with a pairwise loss to learn more discriminative and generalizable features, thus making it appropriate for other related identification tasks like open-set, closed set and verification. We report state-of-the-art accuracy on facial recognition of two primate species, rhesus macaques and chimpanzees under the four protocols of classification, verification, closed-set identification and open-set recognition.

==> Sections/Applications.tex <==
The system for unique identification of individuals contributes in many ways towards the wellbeing of the society and the humans. With the current technological developments that has made hand-held devices like cell phones with cameras affordable to large population, the same can be utilized for citizen science program across the nation. By using a simple application installed on the device, the conflict incidents with geotag information can be reported. This would not only help the officials to track the location of the incident as well as allow them to maintain a centralized database. With access to the huge image database, the population census can be done avoiding field surveys and success of programs like sterilization can be quantified. Furthermore, owing to its applicability across different non human primates, adding the PFID module to widely population wildlife conservation tools like SMART \cite{}, would aid in conservation and monitoring of non human primates. 
% \subsubsection{Citizen Science}
% The overpopulation of macaques

% \subsubsection{Centralized Database and Extensibility} 
% While the software is used to report several incidents, this allows to create a global database of density of population across the country.


% \subsubsection{Troop Level Identification} 
% Identifying individuals aids in population


% \subsection{Monitoring of Endangered Species}

% \subsubsection{Future Integration with Conservation Tool}

% SMART wildlife monitoring 
%  MSTripes

==> Sections/diff_primates.tex <==
a\begin{figure}[h]
% \vspace{-0.5cm}	
	\centering
			{
			\includegraphics[width =0.1\textwidth,height=1cm,keepaspectratio]{Plots/example/Bonnet_macaque_(Macaca_radiata)_head.jpg}
        \includegraphics[width  =0.1\textwidth,height=1cm,keepaspectratio]{Plots/example/Purple-faced-Langur.jpg}
        \includegraphics[width  =0.1\textwidth,height=1cm,keepaspectratio]{Plots/3.jpg}
        \includegraphics[width  =0.1\textwidth,height=1cm,keepaspectratio]{Plots/example/Dry-Zone-Toque-Macaque-012.jpg}
        }
  	\caption{Example of different primates that dwell in urban, semi urban areas.}
		\label{fig: intro_example}
        \vspace{-0.5cm}	
\end{figure}
